CryptoNite: Revealing the Pitfalls of End-to-End Private Inference at Scale

The privacy concerns of providing deep learning inference as a service have underscored the need for private inference (PI) protocols that protect users' data and the service provider's model using cryptographic methods. Recently proposed PI protocols have achieved significant reductions in PI latency by moving the computationally heavy homomorphic encryption (HE) parts to an offline/pre-compute phase. Paired with recent optimizations that tailor networks for PI, these protocols have achieved performance levels that are tantalizingly close to being practical. In this paper, we conduct a rigorous end-to-end characterization of PI protocols and optimization techniques and find that the current understanding of PI performance is overly optimistic. Specifically, we find that offline storage costs of garbled circuits (GC), a key cryptographic protocol used in PI, on user/client devices are prohibitively high and force much of the expensive offline HE computation to the online phase, resulting in a 10-1000$\times$ increase to PI latency. We propose a modified PI protocol that significantly reduces client-side storage costs for a small increase in online latency. Evaluated end-to-end, the modified protocol outperforms current protocols by reducing the mean PI latency by $4\times$ for ResNet18 on TinyImageNet. We conclude with a discussion of several recently proposed PI optimizations in light of the findings and note many actually increase PI latency when evaluated from an end-to-end perspective.

==> additional/case1_tail_latency.tex <==
\begin{figure*}
\centering
\subfloat[ResNet32]{\includegraphics[scale=0.25]{figures/r32_delphi_mean}}
\subfloat[VGG16]{\includegraphics[scale=0.25]{figures/vgg16_delphi_mean}} 
\subfloat[ResNet18]{\includegraphics[scale=0.25]{figures/r18_delphi_mean}}
\caption{Mean latency for ``Server-garbler'' protocol.}
\vspace{-1em}
\label{fig:Case1TailLatency}
\end{figure*}

==> additional/max_sustainable_throughput.tex <==
% \begin{figure*}
% \centering
% \subfloat[ResNet-32]{\includegraphics[scale=0.28]{figures/r32_maximum_sustainable_throughput}} 
% \subfloat[VGG-16]{\includegraphics[scale=0.28]{figures/vgg16_maximum_sustainable_throughput}} 
% \subfloat[ResNet-18]{\includegraphics[scale=0.28]{figures/r18_maximum_sustainable_throughput}}
% \caption{Maximum sustainable throughput for ResNet-32, VGG-16, and ResNet-18 (a, b, and c respectively) evaluated on $32\times32$ image (CIFAR-100/10) over a simulation period of 24 hrs: Initially, at lower arrival rate, number of completed requests linearly increases with arrival rate; however, {\em saturates} beyond a certain arrival rate (called as maximum sustainable throughput) and none of the requests get served. We note that network with higher FLOPs saturates earlier and able to sustain relatively lower arrival rate than the networks with lower FLOPs. Here, the order of maximum sustainable throughput is ResNet-32 $>$ VGG-16 $>$ ResNet-18}
% \label{fig:MaxSustainableThroughput}
% \end{figure*}

==> additional/mean_latency_with_throughput.tex <==



% \begin{figure*}
% \centering
% \subfloat[ResNet-32]{\includegraphics[scale=0.25]{figures/r32_mean_latency_throughput}}
% \subfloat[VGG-16]{\includegraphics[scale=0.25]{figures/vgg16_mean_latency_throughput}} 
% \subfloat[ResNet-18]{\includegraphics[scale=0.25]{figures/r18_mean_latency_throughput}}
% \caption{Mean (PI) latency as a function of arrival rate for ResNet-32, VGG-16, and ResNet-18 (a, b, and c respectively) evaluated on $32\times32$ image (CIFAR-100/10) over a simulation period of 24 hrs: Initially, at lower arrival rate, mean latency is constant and then increases {\em exponentially} and starts saturating (as none of the requests get served) beyond a certain higher arrival rate. We note networks with lower FLOPs are able to accommodate higher arrival rate with constant mean PI latency (here the order is ResNet-32 $>$ VGG-16 $>$ ResNet-18)}
% \vspace{-1em}
% \label{fig:Case2MeanLatency}
% \end{figure*}




==> plots/storage_scaling.tex <==
\begin{figure} [t]
\centering
\includegraphics[scale=0.5]{mlsys2022style/figures/storage_problem_update.pdf}
\caption{Maximum sustainable throughput for ResNet-32, VGG-16, and ResNet-18 (a, b, and c respectively) evaluated on $32\times32$ image (CIFAR-100/10) over a simulation period of 24 hrs: Initially, at lower arrival rate, number of completed requests linearly increases with arrival rate; however, {\em saturates} beyond a certain arrival rate (called as maximum sustainable throughput) and none of the requests get served. We note that network with higher FLOPs saturates earlier and able to sustain relatively lower arrival rate than the networks with lower FLOPs. Here, the order of maximum sustainable throughput is ResNet-32 $>$ VGG-16 $>$ ResNet-18}
\label{fig:StorageScaling}
\end{figure}
